Higher-order semantics for quantum programming languages with classical control

This thesis studies the categorical formalisation of quantum computing, through the prism of type theory, in a three-tier process. The first stage of our investigation involves the creation of the dagger lambda calculus, a lambda calculus for dagger compact categories. Our second contribution lifts the expressive power of the dagger lambda calculus, to that of a quantum programming language, by adding classical control in the form of complementary classical structures and dualisers. Finally, our third contribution demonstrates how our lambda calculus can be applied to various well known problems in quantum computation.

==> ConstituentRelations.tex <==
\begin{landscape}
\thispagestyle{empty}
% %% %%% CRITERIA FOR A CATEGORY
\noindent\textbf{Composition with identity:}
\vskip .1cm
% (right)
$a:A \vdash_S b:B \sim$
\AxiomC{$a:A \vdash_S b:B$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x:B \vdash x:B$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$a:A \vdash_{S \cup \{b:x\}} x:B$}
\DisplayProof

% (left)
\vskip .2cm
$a:A \vdash_S b:B \sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x:A \vdash x:A$}
\AxiomC{$a:A \vdash_S b:B$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$x:A \vdash_{S \cup \{x:a\}} b:B$}
\DisplayProof

% %% %%% CRITERIA FOR A MONOIDAL CATEGORY
\vskip .2cm
\noindent\textbf{Bifunctoriality:}
\vskip .1cm
\hskip -5cm
\def\defaultHypSeparation{\hskip 0.1cm}
\AxiomC{$a:A \vdash_{S_1} b:B$}
\AxiomC{$b^\prime:B \vdash_{S_3} p:P$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$a:A \vdash_{S_1 \cup S_3 \cup \{b:b^\prime\}} p:P$}
\AxiomC{$c:C \vdash_{S_2} d:D$}
\AxiomC{$d^\prime:D \vdash_{S_4} q:Q$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$c:C \vdash_{S_2 \cup S_4 \cup \{d:d^\prime\}} q:Q$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$a:A, c:C \vdash_{S_1 \cup S_2 \cup S_3 \cup S_4 \cup \{b:b^\prime, d:d^\prime\}} p \otimes q:P \otimes Q$}
\DisplayProof
$\sim$
\AxiomC{$a:A \vdash_{S_1} b:B$}
\AxiomC{$c:C \vdash_{S_2} d:D$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$a:A, c:C \vdash_{S_1 \cup S_2} b \otimes d:B \otimes D$}
\AxiomC{$b^\prime:B \vdash_{S_3} p:P$}
\AxiomC{$d^\prime:D \vdash_{S_4} q:Q$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$b^\prime:B, d^\prime:D \vdash_{S_3 \cup S_4} p \otimes q:P \otimes Q$}
\RightLabel{\footnotesize $\bigotimes L$}
\UnaryInfC{$b^\prime \otimes d^\prime:B \otimes D \vdash_{S_3 \cup S_4} p \otimes q:P \otimes Q$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$a:A, c:C \vdash_{S_1 \cup S_2 \cup S_3 \cup S_4 \cup \{b \otimes d:b^\prime \otimes d^\prime\}} p \otimes q:P \otimes Q$}
\DisplayProof
\def\defaultHypSeparation{\hskip .2in}

\vskip .2cm
\noindent\textbf{Associativity pentagon:}
\vskip .1cm
\hskip -1.3cm
\AxiomC{$a:A, b:B, c:C, d:D \vdash_S t:T$}
\UnaryInfC{$a:A, b:B, c \otimes d : C \otimes D \vdash_S t:T$}
\UnaryInfC{$a:A, b \otimes (c \otimes d) : B \otimes (C \otimes D) \vdash_S t:T$}
\DisplayProof
$\sim$
\AxiomC{$a:A, b:B, c:C, d:D \vdash_S t:T$}
\UnaryInfC{$a:A, b \otimes c : B \otimes C, d:D \vdash_S t:T$}
\UnaryInfC{$a:A, (b \otimes c) \otimes d : (B \otimes C) \otimes D \vdash_S t:T$}
\UnaryInfC{$a:A, b \otimes (c \otimes d) : B \otimes (C \otimes D) \vdash_S t:T$}
\DisplayProof

\vskip .2cm
\noindent\textbf{Triangular unit condition:}
\vskip .1cm
\hskip -2cm
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$b:B \vdash b:B$}
\RightLabel{\footnotesize $\lambda_B$}
\UnaryInfC{$1:I, b:B \vdash b:B$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$a:A, 1 \otimes b:I \otimes B \vdash a \otimes b:A \otimes B$}
\DisplayProof
$\sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\RightLabel{\footnotesize $\rho_A$}
\UnaryInfC{$a:A, 1:I \vdash a:A$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$b:B \vdash b:B$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$a:A, 1:I, b:B \vdash a \otimes b:A \otimes B$}
\RightLabel{\footnotesize $\bigotimes L$}
\UnaryInfC{$a:A, 1 \otimes b:I \otimes B \vdash a \otimes b:A \otimes B$}
\DisplayProof

\vskip 1cm
\begin{center}
    37
\end{center}

\newpage
\thispagestyle{empty}

% %% %%% CRITERIA FOR A SYMMETRIC MONOIDAL CATEGORY
\noindent\textbf{Exchange involution:}
\vskip .1cm
$a:A, b:B \vdash a \otimes b:A \otimes B \sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A, b:B \vdash a \otimes b:A \otimes B$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$b:B, a:A \vdash a \otimes b:A \otimes B$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$a:A, b:B \vdash a \otimes b:A \otimes B$}
\DisplayProof

\vskip .2cm
\noindent\textbf{Unit exchange triangle:}
\vskip .1cm
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\RightLabel{\footnotesize $\rho_A$}
\UnaryInfC{$a:A, 1:I \vdash a:A$}
\DisplayProof
$\sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\RightLabel{\footnotesize $\lambda_A$}
\UnaryInfC{$1:I, a:A \vdash a:A$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$a:A, 1:I \vdash a:A$}
\DisplayProof

\vskip .2cm
\noindent\textbf{Exchange hexagon:}
\vskip .1cm
\AxiomC{$c:C, a:A, b:B \vdash_S t:T$}
\RightLabel{\footnotesize $\bigotimes L$}
\UnaryInfC{$c:C, a \otimes b:A \otimes B \vdash_S t:T$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$a \otimes b:A \otimes B, c:C \vdash_S t:T$}
\RightLabel{\footnotesize $\bigotimes L$}
\UnaryInfC{$a:A, b \otimes c:B \otimes C \vdash_S t:T$}
\DisplayProof
$\sim$
\AxiomC{$c:C, a:A, b:B \vdash_S t:T$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$a:A, c:C, b:B \vdash_S t:T$}
\RightLabel{\footnotesize($\bigotimes L$)}
\UnaryInfC{$a:A, c \otimes b:C \otimes B \vdash_S t:T$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$a:A, b \otimes c:B \otimes C \vdash_S t:T$}
\DisplayProof

% %% %%% CRITERIA FOR A COMPACT CLOSED CATEGORY
\vskip .2cm
\noindent\textbf{1st yanking condition:}
\vskip .2cm
\hskip -4cm
{\footnotesize
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x:A \vdash x:A$}
\DisplayProof
$\sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_1:A \vdash x_1:A$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_2:A \vdash x_2:A$}
\RightLabel{\footnotesize Curry}
\UnaryInfC{$1:I \vdash x_{2*} \otimes x_2:A^* \otimes A$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$x_1:A, 1:I \vdash x_1 \otimes (x_{2*} \otimes x_2):A \otimes (A^* \otimes A)$}
\RightLabel{\footnotesize $\rho_A^{-1}$}
\UnaryInfC{$x_1:A \vdash x_1 \otimes (x_{2*} \otimes x_2):A \otimes (A^* \otimes A)$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_3:A \vdash x_3:A$}
\RightLabel{\footnotesize Uncurry}
\UnaryInfC{$x_{3*}:A^*, x_3:A \vdash 1:I$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$x_3:A, x_{3*}:A^* \vdash 1:I$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_4:A \vdash x_4:A$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$x_3:A, x_{3*}:A^*, x_4:A \vdash 1 \otimes x_4:I \otimes A$}
\RightLabel{\footnotesize $\bigotimes L$}
\UnaryInfC{$x_3:A, x_{3*} \otimes x_4:A^* \otimes A \vdash 1 \otimes x_4:I \otimes A$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$x_1:A \vdash_{\{x_1 \otimes (x_{2*} \otimes x_2):x_3 \otimes (x_{3*} \otimes x_4)\}} 1 \otimes x_4:I \otimes A$}
\UnaryInfC{$x:A \vdash 1 \otimes x:I \otimes A$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\RightLabel{\footnotesize $\lambda_A$}
\UnaryInfC{$1:I, a:A \vdash a:A$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$x:A \vdash_{\{1 \otimes x:1 \otimes a\}} a:A$}
\UnaryInfC{$x:A \vdash x:A$}
\DisplayProof
}

\vskip .4cm
\begin{center}
    38
\end{center}

\newpage
\thispagestyle{empty}

\noindent\textbf{2nd yanking condition:}
\vskip .2cm
\hskip -5cm
{\footnotesize
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x:A \vdash x:A$}
\RightLabel{\footnotesize Dual}
\UnaryInfC{$x_*:A^* \vdash x_*:A^*$}
\DisplayProof
$\sim$
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_1:A \vdash x_1:A$}
\RightLabel{\footnotesize Curry}
\UnaryInfC{$1:I \vdash x_{1*} \otimes x_1:A^* \otimes A$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_2:A \vdash x_2:A$}
\RightLabel{\footnotesize Dual}
\UnaryInfC{$x_{2*}:A^* \vdash x_{2*}:A^*$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$1:I, x_{2*}:A^* \vdash (x_{1*} \otimes x_1) \otimes x_{2*}:(A^* \otimes A) \otimes A^*$}
\RightLabel{\footnotesize $\lambda_{A^*}^{-1}$}
\UnaryInfC{$x_{2*}:A^* \vdash (x_{1*} \otimes x_1) \otimes x_{2*}:(A^* \otimes A) \otimes A^*$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_3:A \vdash x_3:A$}
\RightLabel{\footnotesize Dual}
\UnaryInfC{$x_{3*}:A^* \vdash x_{3*}:A^*$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$x_4:A \vdash x_4:A$}
\RightLabel{\footnotesize Uncurry}
\UnaryInfC{$x_{4*}:A^*, x_4:A \vdash 1:I$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$x_4:A, x_{4*}:A^* \vdash 1:I$}
\RightLabel{\footnotesize $\bigotimes R$}
\BinaryInfC{$x_{3*}:A^*, x_4 \otimes x_{4*}:A \otimes A^* \vdash x_{3*} \otimes 1:A^* \otimes I$}
\RightLabel{\footnotesize $\bigotimes L^{-1}$}
\UnaryInfC{$x_{3*}:A^*, x_4:A, x_{4*}:A^* \vdash x_{3*} \otimes 1:A^* \otimes I$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$x_{2*}:A^* \vdash_{\{(x_{1*} \otimes x_1) \otimes x_{2*}:(x_{3*} \otimes x_4) \otimes x_{4*}\}} x_{3*} \otimes 1:A^* \otimes I$}
\UnaryInfC{$x_*:A^* \vdash 1 \otimes x_*:I \otimes A^*$}
\AxiomC{}
\RightLabel{\footnotesize Id}
\UnaryInfC{$a:A \vdash a:A$}
\RightLabel{\footnotesize Dual}
\UnaryInfC{$a_*:A^* \vdash a_*:A^*$}
\RightLabel{\footnotesize $\rho_{A^*}$}
\UnaryInfC{$a_*:A^*, 1:I \vdash a_*:A^*$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$x_*:A^* \vdash_{\{x_* \otimes 1:a_* \otimes 1\}} a_*:A^*$}
\UnaryInfC{$x_*:A^* \vdash x_*:A^*$}
\DisplayProof
}

% %% %%% CRITERIA FOR A DAGGER COMPACT CATEGORY
\vskip .2cm
\noindent\textbf{Dagger involution:}
\vskip .1cm
$a:A \vdash_S b:B \sim$
\AxiomC{$a:A \vdash_S b:B$}
\RightLabel{\footnotesize $\dag$-flip}
\UnaryInfC{$b:B \vdash_{S_*} a:A$}
\RightLabel{\footnotesize $\dag$-flip}
\UnaryInfC{$a:A \vdash_S b:B$}
\DisplayProof

\vskip .2cm
\noindent\textbf{Dagger compact symmetry:}
\vskip .1cm
\AxiomC{$x:A \vdash x:A$}
\RightLabel{\footnotesize Curry}
\UnaryInfC{$\vdash x_* \otimes x:A^* \otimes A$}
\DisplayProof
$\sim$
\AxiomC{$x:A \vdash x:A$}
\RightLabel{\footnotesize Uncurry}
\UnaryInfC{$x_*:A^*, x:A \vdash$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$x:A, x_*:A^* \vdash$}
\RightLabel{\footnotesize $\dag$-flip}
\UnaryInfC{$\vdash x \otimes x_*:A \otimes A^*$}
\AxiomC{$z_*:A^*, y:A \vdash z_* \otimes y:A^* \otimes A$}
\RightLabel{\footnotesize Exchange}
\UnaryInfC{$y:A, z_*:A^* \vdash z_* \otimes y:A^* \otimes A$}
\RightLabel{\footnotesize Cut}
\BinaryInfC{$\vdash_{\{x \otimes x_*:y \otimes z_*\}} z_* \otimes y:A^* \otimes A$}
\UnaryInfC{$\vdash x_* \otimes x:A^* \otimes A$}
\DisplayProof

\vskip 1.5cm
\begin{center}
    39
\end{center}

\end{landscape}

